Confidential Machine Learning Computation in Untrusted Environments: A Systems Security Perspective

As machine learning (ML) technologies and applications are rapidly changing many computing domains, security issues associated with ML are also emerging. In the domain of systems security, many endeavors have been made to ensure ML model and data confidentiality. ML computations are often inevitably performed in untrusted environments and entail complex multi-party security requirements. Hence, researchers have leveraged the Trusted Execution Environments (TEEs) to build confidential ML computation systems. We conduct a systematic and comprehensive survey by classifying attack vectors and mitigation in confidential ML computation in untrusted environments, analyzing the complex security requirements in multi-party scenarios, and summarizing engineering challenges in confidential ML implementation. Lastly, we suggest future research directions based on our study.

==> Makefile <==
# Latex Makefile using latexmk
# Modified by Dogukan Cagatay <dcagatay@gmail.com>
# Originally from : http://tex.stackexchange.com/a/40759
#
# Change only the variable below to the name of the main tex file.
# PROJNAME=$(shell basename $(CURDIR))
PROJNAME=main


# You want latexmk to *always* run, because make does not have all the info.
# Also, include non-file targets in .PHONY so they are run regardless of any
# file of the given name existing.
.PHONY: $(PROJNAME).pdf all clean

# The first rule in a Makefile is the one executed by default ("make"). It
# should always be the "all" rule, so that "make" and "make all" are identical.
all: $(PROJNAME).pdf

# CUSTOM BUILD RULES

# In case you didn't know, '$@' is a variable holding the name of the target,
# and '$<' is a variable holding the (first) dependency of a rule.
# "raw2tex" and "dat2tex" are just placeholders for whatever custom steps
# you might have.

%.tex: %.raw
	./raw2tex $< > $@

%.tex: %.dat
	./dat2tex $< > $@

# MAIN LATEXMK RULE

# -pdf tells latexmk to generate PDF directly (instead of DVI).
# -pdflatex="" tells latexmk to call a specific backend with specific options.
# -use-make tells latexmk to call make for generating missing files.

# -interactive=nonstopmode keeps the pdflatex backend from stopping at a
# missing file reference and interactively asking you for an alternative.

ENGINE=pdflatex

PDFLATEX_OPT="$(ENGINE) -synctex=1 -interaction=nonstopmode -file-line-error --shell-escape"

$(PROJNAME).pdf: main.tex
	latexmk -f  --jobname=$(PROJNAME) -pdf \
	-pdflatex=$(PDFLATEX_OPT) -use-make $<

cleanall:
	rm -rf $(PROJNAME).aux $(PROJNAME).bbl $(PROJNAME).blg $(PROJNAME).fdb_latexmk  \
	$(PROJNAME).fls $(PROJNAME).log $(PROJNAME).out

clean:
	rm -rf *.aux *.bbl \
	*.blg *.fdb_latexmk  \
	*.fls *.log *.out \
	$(PROJNAME).pdf




==> glossaries.tex <==
% \makenoidxglossaries
\glsdisablehyper
\newacronym{ai}{AI}{artificial intelligence}
\newacronym{ml}{ML}{machine learning}
\newacronym{dp}{DP}{differential privacy}
\newacronym{mpc}{MPC}{multi-party computation}
\newacronym{he}{HE}{homomorphic encryption}
\newacronym{tee}{TEE}{trusted execution environment}
\newacronym{mia}{MIA}{membership inference attack}
\newacronym{paas}{PaaS}{prediction as a service}
\newacronym{gemm}{GEMM}{general matrix multiplication}
\newacronym{svm}{SVM}{support-vector machine}
\newacronym{gan}{GAN}{generative adversarial network}
\newacronym{tz}{TZ}{TrustZone}
\newacronym{sgx}{SGX}{Software Guard Extension}
\newacronym{mmu}{MMU}{memory management unit}
\newacronym{cnn}{CNN}{convolutional neural network}
\newacronym{mlaas}{MLaaS}{machine learning as a service}
\newacronym{api}{API}{application programming interface}
\newacronym{mpml}{MPML}{multi-party machine learning}
\newacronym{dnn}{DNN}{deep neural network}
\newacronym{csp}{CSP}{cloud service provider}
\newacronym{gdpr}{GDPR}{General Data Protection Regulation}
\newacronym{fl}{FL}{federated learning}
\newacronym{gpu}{GPU}{graphics processing unit}
\newacronym{em}{EM}{electromagnetic}



==> settings.tex <==
%%%%%% IEEE Access default
%\usepackage{cite}
\usepackage{tikz}
\usepackage{balance}
\usepackage{textcomp}
\usepackage{arydshln}
\usepackage{makecell}

\usetikzlibrary{mindmap}
\RequirePackage{spotcolor}
\NewSpotColorSpace{PANTONE}
\AddSpotColor{PANTONE} {PANTONE3015C} {PANTONE\SpotSpace 3015\SpotSpace C} {1 0.3 0 0.2}
\SetPageColorSpace{PANTONE}

% \definecolor{accessblue}{cmyk}{.24,1,1,0}
% \definecolor{greycolor}{cmyk}{0,0,0,.8}
\definecolor{CustomGreen}{rgb}{0,0.7,0}
\definecolor{CustomBlue}{rgb}{0,0,0.7}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{pifont} % Checkmarks and xmarks
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}


\usepackage{algorithmic}
\usepackage{graphicx}% better graphic
\usepackage{textcomp}
\usepackage{lipsum}  
\usepackage{rotating}  

\usepackage[square,numbers]{natbib}
\usepackage{hypernat}
\usepackage{verbatim}

% \usepackage[dvipsnames]{xcolor}

\newcounter{chalcounter}
\newcommand\chalcnt{\stepcounter{chalcounter}\thechalcounter}

\setcounter{secnumdepth}{6}

% \usepackage{tcolorbox}
\usepackage{soul}

\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
    
%%%%%% Check if draft
\usepackage{ifdraft}

%%%%%% Outline
\usepackage{outlines}


%%%%%% Ref
\usepackage{hyperref}
\hypersetup{
     colorlinks=true,
     citecolor=CustomGreen,      
     linkcolor=CustomBlue,
     urlcolor=black
     }
\usepackage{cleveref}
\crefname{section}{§}{§§}


%%%%%% FIXME & TODO
% \definecolor{fxtarget}{rgb}{0.8000,0.0000,0.0000}

%%%%%% Table
\usepackage{adjustbox} %adjust size of table
\usepackage{siunitx}
\usepackage{makecell}
\usepackage{booktabs,multirow} %Better defaults
\usepackage{multicol}
% \usepackage{soul}
% for underlines
% \usepackage[normalem]{ulem}
%\renewcommand\hl{\bgroup\markoverwith
    % {\textcolor{yellow}{\rule[-.5ex]{.1pt}{2.5ex}}}\ULon}
% \usepackage[table]{xcolor} % for cell colors
\usepackage{changepage,threeparttable} % for wide tables
% \usepackage{fullpage}
\usepackage{threeparttable}
\usepackage{wasysym}
%\usepackage{dingbat}
\usepackage{tabularx}
\usepackage{diagbox}
\usepackage[zerostyle=b,scaled=1]{newtxtt}
\usepackage{fontawesome}

\newcolumntype{C}{>{\centering\arraybackslash}X}
\setlength{\extrarowheight}{1pt}
\renewcommand\theadfont{\normalfont\bfseries} % Make header bold%
% \renewcommand\theadgape{\Gape[0.6ex]}
% \renewcommand\cellgape{\Gape[1pt][0.8cm]}
%\newcommand*{\thead}[1]{%
%\multicolumn{1}{c}{\bfseries\begin{tabular}{@{}c@{}}#1\end{tabular}}}


% Other
\usepackage{xparse}
\usepackage{markdown}
\usepackage{xspace}
\usepackage{listofitems} %Powerful array arguments
\def\foreachitemdeliver#1#2{%
  \begingroup
  \def\foreachitemdeliverpartial{}%
  \def\foreachitemdeliveraction##1{#2}%
  \foreachitem\foreachitemitem\in#1{%
    \edef\foreachitemdeliverpartial{%
      \unexpanded\expandafter{\foreachitemdeliverpartial}%
      \unexpanded\expandafter\expandafter\expandafter{%
        \expandafter\foreachitemdeliveraction\expandafter{\foreachitemitem}%
      }%
    }%
  }%
  \expandafter\endgroup\foreachitemdeliverpartial
}
\newcommand*{\hdr}[1]{\noindent\textbf{#1}\xspace%
    \addcontentsline{toc}{paragraph}{\bfseries#1}}
    
\let\emph\textit


\usepackage{tocloft}
%\renewcommand*{\cftsecdotsep}{4.5}  % use dots in the section entries
\renewcommand*{\cftsecnumwidth}{3em} % increase space for Roman numerals
\renewcommand*{\cftparaindent}{5em} 
\renewcommand*{\cftsubparaindent}{4em} 
\setcounter{tocdepth}{5}
% \newcommand\addtoc[1]{%
%   \refstepcounter{paragraph}%
%   \addcontentsline{toc}{paragraph}{\protect\numberline{\thesection}#1}%
%   \sectionmark{#1}}

\newcommand\addtoc[1]{%
    \addcontentsline{toc}{subparagraph}{{$\hookrightarrow$~\emph{#1}}}%
}

%%% Boxed text
\newcommand{\boxedpar}[1]{\vspace{0.7em}\noindent\fbox{\begin{minipage}{0.97\columnwidth}#1\end{minipage}}\vspace{0.5em}}

%%% Notes
\usepackage{fixme}
% \usepackage{xcolor}
\fxsetup{nomargin,inline,theme=color,author=}
% \colorlet{fxnote}{blue}
\definecolor{fxnote}{rgb}{0.2000,0.2000,0.8000}
\newcommand{\hj}[1]{\textcolor{blue}{HJ: #1}}
\newcommand{\kha}[1]{\textcolor{blue}{KHA: #1}}
\newcommand{\noh}[1]{\textcolor{green}{NOH: #1}}
% \newcommand{\kha}[1]{\fxnote{KHA: #1 (\thesubsection)}}
\newcommand{\fix}[1]{\textcolor{red}{FIX: #1}}
% \newcommand{\fix}[1]{\fxfatal{FIX: #1 (\thesubsection)}}
% \newcommand{\fix}[1]{\fxfatal{FIX: #1 (\thesubsection)}}
\newcommand{\todo}[1]{\fxnote{TODO: #1 (\thesubsection)}}

\newcommand{\sw}[1]{{\color{blue} sw: #1}}
% \newcommand{\id}[1]{\textbf{\texttt{#1}}}
\DeclareRobustCommand{\id}[1]{{\bfseries\ttfamily #1}}




% \newcommand\hl[1]{\colorbox{yellow}{#1}}

\newcommand{\hjcheck}{{\large{\textcolor{CustomGreen}{\faCheck}}}}
\newcommand{\uncheck}{{\large{\textcolor{red}{\faTimes}}}}

\renewcommand{\hl}[1]{#1}

%\newcommand*{\remove}[1]{\st{\hl{#1}}}
%% Circled number
\newcommand{\circled}[1]{\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {\bfseries #1}}}}
\renewcommand\theadset{\def\arraystretch{0.5}}%

\usepackage{tablefootnote}

% \ding{172}--\ding{181} % seriffed fonts
% \ding{192}--\ding{201} % sans-seriffed fonts
% \newcommand*{\circled}[1]{%
%   \stringcases
    % {#1}%
    % {%
    %   {1}{\ding{172}}%
    %   {b}{now this is b}%
    %   {c}{you want me to do c?}%
    % }%
    % {[nada]}%
% }

%\newcommand*\circled[1]{\tikz[baseline=(char.base)]{ \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}

% Draw circle
% \newcommand*\emptycirc[1][1ex]{\tikz\draw (0,0) circle (#1);} 
% \newcommand*\halfcirc[1][1ex]{%
%   \begin{tikzpicture}
%   \draw[fill] (0,0)-- (90:#1) arc (90:270:#1) -- cycle ;
%   \draw (0,0) circle (#1);
%   \end{tikzpicture}}
% \newcommand*\fullcirc[1][1ex]{\tikz\fill (0,0) circle (#1);} 

\newcommand{\showissue}{}
\ifdefined\showissue
\else
\fi


% Acronym & Glossary
\usepackage{glossaries-extra}
\glsdisablehyper
\defglsdisplayfirst[\glsdefaulttype]{\textit{#1}}
\setabbreviationstyle[acronym]{long-short}
\input{glossaries}


==> tables/multi-party.tex <==
\begin{table*}[htbp]
    \centering
    \newcolumntype{Y}{>{\centering\arraybackslash}X}
    \newcolumntype{M}{>{\hsize=0.5\hsize\centering\arraybackslash}X}
    \newcolumntype{S}{>{\hsize=0.20\hsize\centering\arraybackslash}X}
    \begin{tabularx}{\textwidth}{>{\hsize=1.3\hsize}XSSSSSSSSSSSSS}
       \toprule
       & \multicolumn{3}{c}{\thead{Scenario}} & \multicolumn{3}{c}{\thead{Protected Assets}} & \multicolumn{2}{c}{\thead{Computation}} & \multicolumn{5}{c}{\thead{Attacker Capabilities}}&\\
       \cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-9} \cmidrule(lr){10-14}
       \thead{Scenario}  & \thead{\id{E-1}} &  \thead{\id{E-2}} & \thead{\id{E-3}} & \id{P-1}&\id{P-2} &\id{P-3} & \id{C-1} & \id{C-2} & \id{AC-1} & \id{AC-2} & \id{AC-3} & \id{AC-4} & \id{AC-5}\\
       \midrule
        Ohrimenko et al. \cite{ohrimenko2016oblivious}  & \checkmark & \checkmark & \checkmark &\checkmark & \checkmark&\checkmark & \checkmark & \checkmark &\checkmark & \checkmark & & \checkmark & \checkmark \\
       \bottomrule
    \end{tabularx}
    \caption{Multi-party ML scenarios by protected assets and attacker model. Different security requirements from different participating parties is the unique characteristic of multi-party ML computation scenarios. The table shows protected assets vs. attackers for each point of view in multi-party ML scenarios. }
    \label{tab:ai_scenario}
\end{table*}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

